Fairness Certification for Natural Language Processing and Large Language Models

Natural Language Processing (NLP) plays an important role in our daily lives, particularly due to the enormous progress of Large Language Models (LLM). However, NLP has many fairness-critical use cases, e.g., as an expert system in recruitment or as an LLM-based tutor in education. Since NLP is based on human language, potentially harmful biases can diffuse into NLP systems and produce unfair results, discriminate against minorities or generate legal issues. Hence, it is important to develop a fairness certification for NLP approaches. We follow a qualitative research approach towards a fairness certification for NLP. In particular, we have reviewed a large body of literature on algorithmic fairness, and we have conducted semi-structured expert interviews with a wide range of experts from that area. We have systematically devised six fairness criteria for NLP, which can be further refined into 18 sub-categories. Our criteria offer a foundation for operationalizing and testing processes to certify fairness, both from the perspective of the auditor and the audited organization.

==> 0-abstract.tex <==
\begin{abstract}
Natural Language Processing (NLP) plays an important role in our daily lives, particularly due to the enormous progress of Large Language Models (LLM). However, NLP has many fairness-critical use cases, e.g., as an expert system in recruitment or as an LLM-based tutor in education. Since NLP is based on human language, potentially harmful biases can diffuse into NLP systems and produce unfair results, discriminate against minorities or generate legal issues. Hence, it is important to develop a fairness certification for NLP approaches.

We follow a qualitative research approach towards a fairness certification for NLP. In particular, we have reviewed a large body of literature on algorithmic fairness in academia and business, and we have conducted semi-structured expert interviews with a wide range of experts from that area. We have systematically devised six fairness criteria for NLP, which can be further refined into 18 sub-categories. Our criteria offer a foundation for operationalizing and testing processes to certify fairness, both from the perspective of the auditor and the audited organization.

% Natural Language Processing (NLP) systems have gained an impactful role in society, particularly, after the widespread adoption of Large Language Models (LLM). Use cases of NLP systems include fairness-critical applications like hiring or education. Human language represents potentially harmful biases that can diffuse into NLP systems. Hence, it makes sense to assess the fairness of such systems independently by a third party via certification. This work builds on the increased attention put on fairness audits in academia. NLP fairness certification is still poorly defined and lacks a meticulous approach for effectively and holistically assessing the fairness of a system. The knowledge gap about contents, sources, and certification processes for the fairness of NLP systems needs to be filled. By conducting expert interviews (N = 14), this work shows criteria for contents and processes that characterize fairness certification for NLP systems. We are the first to offer a holistic scheme of 6 criteria on the highest hierarchy level and 18 on the second hierarchy level for holistic fairness certification of a NLP system. These criteria offer a foundation for operationalizing and testing processes to certify fairness.
\end{abstract}

